pCAMP: Performance Comparison of Machine Learning Packages on the Edges

Machine learning has changed the computing paradigm. Products today are built with machine intelligence as a central attribute, and consumers are beginning to expect near-human interaction with the appliances they use. However, much of the deep learning revolution has been limited to the cloud. Recently, several machine learning packages based on edge devices have been announced which aim to offload the computing to the edges. However, little research has been done to evaluate these packages on the edges, making it difficult for end users to select an appropriate pair of software and hardware. In this paper, we make a performance comparison of several state-of-the-art machine learning packages on the edges, including TensorFlow, Caffe2, MXNet, PyTorch, and TensorFlow Lite. We focus on evaluating the latency, memory footprint, and energy of these tools with two popular types of neural networks on different edge devices. This evaluation not only provides a reference to select appropriate combinations of hardware and software packages for end users but also points out possible future directions to optimize packages for developers.

==> 0Abstract.tex <==
% \subsection*{Abstract}
% Machine Learning has changed the computing paradigm. Products of today are built with machine intelligence as a central attribute, and consumers are beginning to expect near-human interaction with the appliances they use.
% However, much of the deep learning revolution has been limited to the cloud.
% % Enabled by popular toolkits such as Caffe, TensorFlow, and MxNet, and by specialized hardware such as TPUs. 
% Recently, several machine learning frameworks based on edge device were announced, which aim to dramatically reduce the barrier to entry for edge computing. However, there are little researches evaluating these packages on the edges, making it difﬁcult for end users to select an appropriate pair of software and hardware.
% %which lead to a problem that researchers do not know which frameworks are suitable for their experiments.
% % With the burgeoning of AI-based applications developed, should support a variety of artificial intelligence algorithms and models. However, the edge node is not a good fit for executing large scale models since they require large footprints on both the storage and computing power.
% % Deep learning has been shown as a successful machine learning method for a variety of tasks, and its popularity results in numerous open-source deep learning packages.
% % coming to public. Training a deep network is usually a very time-consuming process.
% % To address the huge computational challenge in deep learning, many tools exploit hardware features such as multi-core CPUs and many-core GPUs to shorten the training and inference time. 
% % However, different tools exhibit different features and running performance when they train different types of deep networks on different hardware platforms, making it difﬁcult for end users to select an appropriate pair of software and hardware. 
% In this paper, we make a performance comparison of several state-of-the-art machine learning packages on the edges, including TensorFlow, Caffe2, MXNet, PyTorch, TensorFlow Lite, and CoreML. We focus on evaluating the latency, memory footprint and energy of these tools with two popular types of neural networks on different edge devices. 
% This evaluation can not only provide a reference to select appropriate hardware platforms and software tools for end users, but also points out the possible future directions to optimize the packages for developers.

==> 5insight.tex <==
% \section{Insights}\label{sec:Insight}

% Based on our analysis of the results, we deduces a list of insights and group them into the following categories.



% \subsection{No single winner, each has its merits}
% Figure \ref{fig:performance comparison} presents that there are no obvious single winners on every metric of all hardware platforms, but each has its merits. We list the packages which have the best performance in different cases in \ref{table: best packages}. 
% The first three rows represent the best packages when running AlexNet and the last three rows list the best ones on SqueezeNet. We summarize the merits of every package and provide a reference to select appropriate packages for end users:

% \begin{enumerate}[1)]
% \item TensorFlow runs faster on large-scale models while MXNet and PyTorch spend the least time when running small-scale models.
% \item PyTorch uses the least memory footprint on MacBook and Intel FogNode for large-scale models. Caffe2 is the best memory saving packages for small-scale models.
% \item PyTorch is the most energy efficient package on JetsonTX2. MXNet consumes the least energy when running the small-scale model on MacBook and Intel FogNode.
% \end{enumerate}









% \subsection{Loading models spend more time than running}

% To profile where the time spends, we divide the whole process of running the trained model into several parts and collect the time that each part spends: 1. import the package from disk to memory, 2. load model from disk to memory, 3. first load image from disk to memory, 4. first inference, 5. second load image from disk to memory, 6. second inference, and 7. inference for 100 times.

% As PyTorch performs best when running models on JetsonTX2, we take it as an example. Table \ref{table:time profiling} presents the time of every part spends when leverages PyTorch to execute the inference task on Jetson TX2. Running AlexNet and SqueezeNet spends 11024ms and 7916 ms, respectively, which is much larger than running reference for 100 times.

% The time that spends to load models is larger than run the model for most packages, which implies that there exist some opportunities to further optimize the performance on the edges by decrease the loading latency and decrease the loading frequency.

% \begin{table}[!htp]
% \centering
% \caption{The best packages in different cases}
% \label{table: best packages}
% \begin{tabular}{@{}c|cccc@{}}
% \toprule
% Hardwares & \begin{tabular}[c]{@{}c@{}}Inference\\ time\end{tabular} & All time & Memory  & Energy  \\ \midrule
% MacBook   & Caffe2                                                   & PyTorch  & PyTorch & PyTorch \\
% Fognode   & TensorFlow                                               & MXNet    & PyTorch & PyTorch   \\
% JetsonTX2 & TensorFlow                                               & PyTorch  & Caffe2  & PyTorch \\ \midrule
% MacBook   & MXNet                                                    & MXNet    & Caffe2  & MXNet   \\
% Fognode   & MXNet                                                    & MXNet    & Caffe2  & MXNet   \\
% JetsonTX2 & PyTorch                                                  & PyTorch  & Caffe2  & PyTorch \\ \bottomrule
% \end{tabular}
% \end{table}


% \begin{table}[!htp]
% \centering
% \caption{Time profile of PyTorch on JetsonTX2}
% \label{table:time profiling}
% \begin{tabular}{@{}lll@{}}
% \toprule
%                     & SqueezeNet (ms) & AlexNet (ms) \\ \midrule
% import              & 819             & 757                            \\
% load model          & \textbf{7916}            & \textbf{11024}                          \\
% first load image    & 49              & 47.6                           \\
% first inference     & \textbf{2361}            & \textbf{3038}                           \\
% second load image   & 24              & 21                             \\
% second inference    & 25              & 22                             \\
% inference 100 times & \textbf{1270}            & \textbf{1400}                           \\
% total time            & 12460            & 16318                           \\ \bottomrule
% \end{tabular}
% \end{table}


% \subsection{The tradeoff between memory footprint and latency}
% % \textbf{The tradeoff between memory footprint and latency}

% Analyzing Figure \ref{fig:Inference time} and Figure \ref{fig:Memory footprint}, we observe that these packages favor tradeoff between memory footprint and latency on JetsonTX2. On AlexNet, the inference time of TensorFlow and PyTorch are much shorter than Caffe2, while their utilized more memory. On SqueezeNet, PyTorch also has the same performance. So we believe that TensorFlow and PyTorch sacrifice space to improve efficiency, which can be a useful optimized method for executing the real-time tasks on the edges. 



% % Runtime Breakdown of Interence Task
